Simple Construction of Greedy Trees and Greedy Permutations

\begin{abstract} Greedy permutations, also known as Gonzalez Orderings or Farthest Point Traversals are a standard way to approximate $k$-center clustering and have many applications in sampling and approximating metric spaces. A greedy tree is an added structure on a greedy permutation that tracks the (approximate) nearest predecessor. Greedy trees have applications in proximity search as well as in topological data analysis. For metrics of doubling dimension $d$, a $2^{O(d)}n\log n$ time algorithm is known, but it is randomized and also, quite complicated. Its construction involves a series of intermediate structures and $O(n \log n)$ space. In this paper, we show how to construct greedy permutations and greedy trees using a simple variation of an algorithm of Clarkson that was shown to run in $2^{O(d)}n\log \Delta$ time, where the spread $\spread$ is the ratio of largest to smallest pairwise distances. The improvement comes from the observation that the greedy tree can be constructed more easily than the greedy permutation. This leads to a linear time algorithm for merging two approximate greedy trees and thus, an $2^{O(d)}n \log n$ time algorithm for computing the tree. Then, we show how to extract a $(1+\frac{1}{n})$-approximate greedy permutation from the approximate greedy tree in the same asymptotic running time. \end{abstract}

==> apx_fvd_properties.tex <==
\subsection{Properties of FVDs Constructed Using Clarkson's Algorithm}
\label{apx:fvd_properties}

In this section we give some properties of the FVDs constructed using $\CLARKSON(P, \lazy, \vorapx, \greedy)$ described in Section~\ref{sec:simple_clarkson}.

\begin{restatable}{lem}{degreebound}[Degree Bound Lemma]\label{lem:degree_bound}
    The number of neighbors of a cell in an FVD constructed running $\CLARKSON(P, \lazy, \vorapx, \greedy)$ is at most $(12\vorapx\greedy)^d$.
\end{restatable}
% \degreebound*
\begin{proof}
    Let $\emin$ be the minimum insertion distance among the sites inserted so far.
%    So, for any site $p$, its neighbors are $(\emin/\vorapx)$-packed.
%    It follows that, the out-radius of every site is at most $\emin$.
    Then, the sites are $(\emin/\vorapx)$-packed.
    By the Heap Invariant, the out-radius of every cell is at most $\greedy\emin$.
%    The sites are inserted in a greedy fashion from $\vorapx$-approximate cells.
    The pruning condition guarantees that the distance from $p$ to any neighbor $q$ is bounded as follows.
    \[
        \dist(p,q) \le \outradius(p) + \outradius(q) + \max\{\outradius(p), \outradius(q)\}\le 3\greedy\emin.
    \]
    So, by the Standard Packing Lemma (Lemma~\ref{lem:std_packing}) the number of neighbors is at most $(12 \vorapx\greedy)^d$.
\end{proof}

\begin{lemma}\label{lem:cell_scaling}
    Let $p \in \vor(p')$ in an FVD constructed running $\CLARKSON(P, \lazy, \vorapx, \greedy)$.
    When $p$ is inserted as a site, the cell out-radius, $\outradius(p) \le \frac{\greedy}{\lazy} \dist(p,p')$.
\end{lemma}
\begin{proof}
    Suppose $q \in \vor(q')$ and it moved to $\vor(p)$ when $p$ was inserted from $\vor(p')$.
    It follows that,
    \begin{align*}
        \outradius(p) &\le \dist(p, q) & \because{definition of out-radius}\\
                        &\le \frac{1}{\lazy} \dist(q,q') & \because{$\lazy$-Lazy Moves} \\
                        &\le \frac{\greedy}{\lazy} \dist(p,p') &\because{by the $\greedy$-heap invariant}. &&\qedhere
    \end{align*}
\end{proof}

\begin{lemma}\label{lem:aspect_ratio_bound}[Aspect Ratio Lemma]
    The aspect ratio of a cell in an FVD constructed running $\CLARKSON(P, \lazy, \vorapx, \greedy)$ is at most $\frac{\vorapx\greedy(1+\vorapx)}{\lazy}$.
\end{lemma}
\begin{proof}    
    The out-radius of a cell is maximized when the point is first inserted.
    It will suffice to prove the aspect ratio is bounded for a site $p$ when it is first inserted and also every time the in-radius decreases.
    
    Let $p$ be any site.
    When $p$ is inserted from $\vor(p')$, let $q\in \vor(q')$ be the point such that $\inradius(p) = \dist(p,q)$.
    Then, after the insertion, we have
    \begin{align*}
            \outradius(p)
            &\le \frac{\greedy}{\lazy}\dist(p,p') & \because{Lemma~\ref{lem:cell_scaling}}\\
            &\le \frac{\vorapx\greedy}{\lazy}\dist(p, q') & \because{by the Cell Invariant}\\
            &\le \frac{\vorapx\greedy}{\lazy}(\dist(p,q) + \dist(q,q')) & \because{by the Triangle Inequality}\\
            &\le \frac{\vorapx\greedy(1+\vorapx)}{\lazy}\dist(p,q) & \because{by the Cell Invariant}\\
            &\le \frac{\vorapx\greedy(1+\vorapx)}{\lazy}\inradius(p). & \because{by the choice of $q$}\\
    \end{align*}
    
    The out-radius and in-radius can only decrease as more sites are inserted.
    Decreasing the out-radius will also decrease the aspect ratio, so we need not consider that case.
    If inserting some $q''\in \vor(q')$ causes a point $p''\in \vor(p)$ to move out of the cell so that $\inradius(p) = \dist(p,p'')$, then
    \begin{align*}
        \outradius(p)
            &\le \greedy\,\dist(q',q'')& \because{$\greedy$-heap invariant}\\
            &\le \vorapx\greedy\, \dist(p,q'')& \because{by the Cell Invariant}\\
            &\le \vorapx\greedy(\dist(p,p'') + \dist(p'',q''))& \because{by the Triangle Inequality}\\
            &\le \vorapx\greedy\left(1 + \frac{1}{\lazy}\right)\dist(p,p'')& \because{$\lazy$-Lazy Moves}\\
            &= \frac{\vorapx\greedy(1+\lazy)}{\lazy}\inradius(p). & \because{by the choice of $p''$}\\
            &\le \frac{\vorapx\greedy(1+\vorapx)}{\lazy}\inradius(p). & \because{because $\vorapx \ge 1$} && \qedhere
    \end{align*}
\end{proof}

We refer to $\aspect := \frac{\vorapx\greedy(1+\vorapx)}{\lazy}$ as the aspect ratio bound.

\begin{lemma}\label{lem:fvd_insertion_order}
    The insertion order of sites in $\CLARKSON(P, \lazy, \vorapx, \greedy)$ is $\vorapx\greedy$-greedy.
\end{lemma}
\begin{proof}
    Let $S$ denote the sites just before the insertion of $a \in \vor(a')$.
    It is sufficient to show that $\dist(p, S) \le \vorapx\greedy\dist(a, S)$ for any point $p$.

    Let $p \in \vor(p')$.
    We have,
    \begin{align*}
        \dist(p, S) &\le \dist(p, p')\\
                        &\le \outradius(p') &\because{definition of out-radii}\\
                        &\le \greedy \dist(a, a')  &\because{by the Heap Invariant} \\
                        &\le \greedy \vorapx \dist(a, S) & \because{the Cell Invariant}&&\qedhere
    \end{align*}
\end{proof}

% \begin{theorem}
%     Let $G$ be the greedy tree constructed by $\CLARKSON(P, \lazy, \vorapx, \radapprox)$.
%     Then $G$ is an $(\frac{\lazy}{\radapprox}, \vorapx, \vorapx\radapprox)$-greedy tree.
% \end{theorem}
% \begin{proof}
%     By Lemma~\ref{lem:cell_scaling}, $G$ is $\frac{\lazy}{\radapprox}$-scaling.
%     By Lemma~\ref{lem:fvd_insertion_order}
% \end{proof}

% \begin{proof}
%     Let $P_a$ denote the sequence of sites just before the insertion of $a$ in $\CLARKSON(P, \lazy, \vorapx, \radapprox)$.
%     Let $a = \nodecenter{x}$, where $x \in \vor(q)$, be the next point chosen to be a site.
%     Let $p \in \points(x')$ and $x' \in \vor(q')$.
%     It is sufficient to show that $\dist(p, P_a) \le \vorapx\radapprox \dist(a, P_a)$

%     We have,
%     \begin{align*}
%         \dist(p, P_a) &\le \dist(p, q')\\
%                         &\le \dist(p, \nodecenter{x'}) + \dist(\nodecenter{x'}, q') &\because{Triangle Inequality} \\
%                         &\le \radapprox\dist(\nodecenter{x'}, q') &\because{$\radapprox$-tidy Cells} \\
%                         &\le \vorapx\radapprox \dist(a, P_a)  &\because{Cell Invariant} &&\qedhere
%     \end{align*}
% \end{proof}



